Flow-of-Action: SOP Enhanced LLM-Based Multi-Agent System for Root Cause Analysis

In the realm of microservices architecture, the occurrence of frequent incidents necessitates the employment of Root Cause Analysis (RCA) for swift issue resolution. It is common that a serious incident can take several domain experts hours to identify the root cause. Consequently, a contemporary trend involves harnessing Large Language Models (LLMs) as automated agents for RCA. Though the recent ReAct framework aligns well with the Site Reliability Engineers (SREs) for its thought-action-observation paradigm, its hallucinations often lead to irrelevant actions and directly affect subsequent results. Additionally, the complex and variable clues of the incident can overwhelm the model one step further. To confront these challenges, we propose Flow-of-Action, a pioneering Standard Operation Procedure (SOP) enhanced LLM-based multi-agent system. By explicitly summarizing the diagnosis steps of SREs, SOP imposes constraints on LLMs at crucial junctures, guiding the RCA process towards the correct trajectory. To facilitate the rational and effective utilization of SOPs, we design an SOP-centric framework called SOP flow. SOP flow contains a series of tools, including one for finding relevant SOPs for incidents, another for automatically generating SOPs for incidents without relevant ones, and a tool for converting SOPs into code. This significantly alleviates the hallucination issues of ReAct in RCA tasks. We also design multiple auxiliary agents to assist the main agent by removing useless noise, narrowing the search space, and informing the main agent whether the RCA procedure can stop. Compared to the ReAct method's 35.50% accuracy, our Flow-of-Action method achieves 64.01%, meeting the accuracy requirements for RCA in real-world systems.

==> relatedwork.tex <==
\subsection{Traditional Methods}

The traditional RCA methods can be categorized into four types based on the data modalities they utilize: (1) Metric-based Methods \citep{metric1,metric2,metric3,metric4}: These typically involve constructing bayesian causal networks or graphs using data such as Remote Procedure Call (RPC). RCA is then performed through techniques like random walks or counterfactual analysis on these networks or graphs. (2) Log-based Methods \citep{log1,log2}: These focus on analyzing log data, such as examining changes in log templates or extracting specific keywords. These approaches aim to detect anomalies and simultaneously identify root causes. (3) Trace-based Methods \citep{yu2021microrank,trace2}: These methods identify root causes by observing changes in trace patterns. For instance, MicroRank \citep{yu2021microrank} compares trace distributions before and after a failure to calculate anomaly scores. SparseRCA \citep{yaosparserca} employs historical data to train pattern recognition models for root cause identification. (4) Multi-modal Methods \citep{yao2024chain,yu2023nezha}: These approaches posit that each data modality can, to some degree, reflect the root cause. It typically involves converting all data modalities into events or alerts, constructing a graph, and applying algorithms like PageRank \citep{page1999pagerank} to localize the root cause.


\subsection{LLM-based Methods}

Due to its powerful natural language analysis and reasoning capabilities, LLMs have gradually been applied in RCA. \citet{chen2024automatic} utilizes LLMs for summarization and recalls historically similar incidents to deduce the root cause of current issues. RCAgent \citep{wang2023rcagent} leverages code and log data to construct an agent based on ReAct for automated orchestration in root cause localization. mABC \citep{zhang2024mabc} adopts a more rational multi-agent framework and introduces a blockchain-based voting mechanism among agents. D-Bot \citep{zhou2024d-bot} similarly employs a multi-agent framework, refining tool selection and knowledge structure. However, these methods are predominantly designed for specific scenarios such as databases, incorporating many context-specific elements like agent categories, thereby limiting their generalizability and transferability.
